A Distributional Approach to Controlled Text Generation

We propose a Distributional Approach for addressing Controlled Text Generation from pre-trained Language Models (LMs). This approach permits to specify, in a single formal framework, both "pointwise" and "distributional" constraints over the target LM -- to our knowledge, the first model with such generality -- while minimizing KL divergence from the initial LM distribution. The optimal target distribution is then uniquely determined as an explicit EBM (Energy-Based Model) representation. From that optimal representation we then train a target controlled Autoregressive LM through an adaptive distributional variant of Policy Gradient. We conduct a first set of experiments over pointwise constraints showing the advantages of our approach over a set of baselines, in terms of obtaining a controlled LM balancing constraint satisfaction with divergence from the initial LM. We then perform experiments over distributional constraints, a unique feature of our approach, demonstrating its potential as a remedy to the problem of Bias in Language Models. Through an ablation study, we show the effectiveness of our adaptive technique for obtaining faster convergence. (Code available at https://github.com/naver/gdc)

==> sections/introduction.previous.tex <==
\section{Introduction}


%\paragraph{Controlling a pretrained language model}
Language models (LMs), in a strict sense such as GPT-2/3 \citep{radford2019language,Brown2020LanguageMA}, or an extended sense, such as BERT \citep{devlin-etal-2019-bert}, pretrained on huge amounts of text, have become pre-eminent in NLP. They are typically seen as stores of generic knowledge that can be used for  downstream tasks through fine-tuning, often done by providing a small amount of task-specific training data and extending or modifying the parameters of the pretrained models.

In this paper, we are concerned with the problem of exploiting a generic pretrained LM $a(x)$ over text sequences $x$ (the autoregressive model GPT-2 in our experiments) for obtaining another ``target'' LM $p(x)$ satisfying certain desiderata. For instance, we may want to avoid toxic content; or to prevent certain demographic biases; or to encourage generated texts to speak about sports. 
% or to probe the ``beliefs'' of the model in a certain discourse area by orienting the generic LM towards generating texts in that area.

We propose to formalize this problem as a constraint satisfaction problem over the distribution $p$, by constraining the expectations of certain features, relative to $p$, to have certain values; for instance we would like all the generated texts to speak about sports, and 50\% of them to mention female characters. However, constraints alone underspecify the distribution $p$. We then add the requirement that the KL divergence between $p$ and the pretrained model $a$ be as small as possible while respecting the constraints. This has the consequence that $p$ is now uniquely determined and inherits favorable linguistic qualities from $a$.

The merits of our work can be summarized as follows:
%\begin{itemize}[noitemsep,topsep=0pt,parsep=5pt,partopsep=0pt,leftmargin=*]
\begin{itemize}[noitemsep,topsep=0pt,parsep=5pt,partopsep=0pt,leftmargin=5mm]
%\begin{itemize}[noitemsep,topsep=0pt,parsep=5pt,partopsep=0pt]
\item We introduce a Distributional view for controlled text generation and its formalization as a constraint satisfaction problem coupled with a divergence minimization objective, providing a single framework both for ``distributional'' constraints (collective statistical requirements) and for ``pointwise'' constraints (hard requirements on every individual). To our knowledge, this is the first framework with such generality for controlled text generation. By relying on Information Geometry theory, we show the existence of a unique optimal distribution in exponential family form, a special case of an Energy-Based Model (EBM) 
\textbf{(\S\ref{sec:constraints2ebm})}.
%\textbf{(\S\ref{sec:constraints-2-ebm})}.
\item  We propose the KL-Adaptive DPG algorithm --- a variant of
\citep{opt-rl-arxiv-2019} 
% \citep{opt-rl-arxiv-2019,A-parshakova-etal-2019-global} 
tailored for this problem --- for approximating this optimal EBM distribution by an autoregressive policy \textbf{(\S\ref{sec:ebm-2-policy})}, and show the effectiveness of this adaptive technique in obtaining faster convergence  \textbf{(\S\ref{sec:appendix:exp-ablation})}.\footnote{In the sequel, \S A, \S B ... refer to sections in the Appendix.}
%
\item We conduct experiments in a number of pointwise and distributional conditions, assessing results in terms of divergence from GPT-2, fluency and diversity, with better performance than a number of strong baselines. The distributional experiments show the potential of our approach as a remedy to the current and important problem of bias in pretrained language models, providing a novel direction for addressing these \textbf{(\S\ref{sec:EXPERIMENTS})}. %\textbf{(\S\ref{sec:exp-distributional})}.
%
\end{itemize}






\iffalse %8-pages-constraint

How can we formally express such desiderata over $p(x)$? In a few cases, it is easy. For instance, if we wish to condition the target LM to produce texts starting with a prefix such as ``To prepare pancakes, you ...'', then we just need to prime the generic model with this prefix, and continue generating from there, a technique that is often used. In other cases, it is much more difficult. For example, we may want to only generate sentences that meet a certain general $0/1$ condition not of the ``prefix type'', for instance sentences predicted by a binary classifier to be mentioning climate-change --- we will call such conditions that operate at the level of an individual text \emph{pointwise constraints}. Or suppose we still want to produce texts about climate-change, but whereas such texts from the generic model mention Northern countries 80\% and Southern countries 20\% of the time, we also wish to change these proportions in the target LM to 40\% and 60\% --- such conditions that operate on a group level are referred to as \emph{distributional constraints}.

\paragraph{From Distributional Constraints to Energy Based Model}  One powerful generic way to evaluate the adequacy of a probability distribution $p(x)$ to one's objectives consists in estimating the values (aka ``moments") of the expectations relative to this distribution of a few well-chosen random variables (aka ``features") and to check whether these values fit one's original expectations (in a non-technical sense...).
This is a wide-ranging method, which can also be applied (as few other methods can) to testing the hypothesis that two random samples come from the same distribution (for a general form of this method, see \citep{Gretton2007-MMD}).
%
In this work, we \emph{reverse} this process and use these random variables and their expectations as \emph{first-class objectives} (``moment constraints'') in the design of a target controlled distribution over textual sequences.
%\MDFN{One may note, here or elsewhere in the writing, that a GAN discriminator (or any other discriminator, actually) could be used as a random variable to fit to the data in our framework.} \MKFN{I feel that the GAN comment here is a bit off-context. But I am not sure.}

Moment constraints
%\HEFN{not so clear what is expectation constraints}
are quite powerful, but they have two major defects:
(1) they severely under-specify the target distribution $p(x)$ --- in general, a great many distributions, especially on high-dimensional data such as sequences, can fit a finite number of moment constraints; 
%
(2) they do not explicitly refer to the pretrained model $a(x)$, meaning $p$ cannot exploit $a$ regarding fluency or semantic adequacy. \HEFN{maybe add a hint on why respecting original model prevents degeneration, what previous work did to do that. KL penality. Also maybe mention that GPT-x models costs lot to train so divergence a lot from it is undesirable in the global view not on evaluation from a specific point of view.}

We solve both issues simultaneously by reformulating the problem as one of finding a $p$ of \emph{minimal KL divergence} $\KL(p,a)$ from $a$ that satisfies the constraints. As we will explain, this formulation is a variant of the \emph{Maximum Entropy Principle} inside Information Geometry \citep{Nielsen-intro-information-geometry}, and leads to a unique solution $P(x)$. $P(x)$ is an unnormalized distribution, aka an EBM (Energy Based Model), of which $p(x) =1/Z\ P(x)$ is the normalized version, where $Z \doteq \sum_x P(x)$ is $P$'s partition function. 

\paragraph{From Energy Based Model to Autoregressive Policy} Computing the EBM representation $P$ is a crucial step, as it fully determines the \emph{optimal} distribution $p$ we are looking for. 
However, it is not the end of the story. There are two issues. First, in order to compute $p(x)$, we must compute $Z$, which can be challenging. Second, and even more seriously, even if we know $Z$, we are not able to directly \emph{sample} from $p$.\footnote{Similarly, we would not be able to \emph{optimize} from $p$, i.e. find $\argmax_x p(x)$: knowing an objective function is a far cry from being able to find its maximum.}

These issues are actually central to the whole field of EBMs, which much research devoted to solving them, or to find non-probabilistic alternatives for training and inferring with them \citep{lecun_tutorial_2006}. Here, we stay inside the probabilistic paradigm and want to actually sample from $p$. One possible approach then would be to employ MCMC techniques, 
%such as Metropolis-Hastings 
\citep{Robert:2005:MCS:1051451}. These come with theoretical convergence guarantees in the limit --- i.e. obtaining a sampler producing $x$'s according to a distribution $q_{\text{MCMC}}$ approximating $p$ to an arbitrary precision --- but in practice convergence can be very difficult to assess, and furthermore, obtaining samples can be extremely slow.

By contrast, our objective is to produce an autoregressive ``policy'' (aka  LM) $\pit$ that can be used at inference time as an efficient sampler.%
%
\footnote{Policy-based samplers have an additional important advantage over MCMC-based samplers: they are \emph{explicit} in the sense that for any $x$, the value of $\pit(x)$ can be directly obtained, while (perhaps counter-intuitively) this is not the case for $q_{\text{MCMC}}(x)$, making the use of policies much better suited for adaptive algorithms such as the ones we are considering below.}
%
To this end, we introduce \emph{KL-adaptive DPG (Distributional Policy Gradient)}, a variant of an algorithm recently proposed in \citep{opt-rl-arxiv-2019}. 
%\HEFN{rephrase to highlight our "KL Adaptive DPG" to highlight our work than parshakova etal.}
%
This algorithm trains the policy $\pit$ to approximate $p$ in an adaptive way, namely by capitalizing on gradually improved approximations to provide proposals improving the next round of approximations. At the end of this process, we obtain a final $\pit$ for which we can estimate diverse metrics, including $\KL(p,\pit)$, measuring the approximation quality of $\pit$ relative to the optimal $p$
and $\KL(\pit,a)$, measuring the divergence of $\pit$ relative to $a=$ GPT-2.
%

This two-step approach differs from much research in NLP-oriented work with EBMs, which tends to use EBM representations \emph{inside} the training loops of neural networks, blurring different dimensions of the problem. By contrast --- similarly to \cite{A-parshakova-etal-2019-global,opt-rl-arxiv-2019} in a different context --- we clearly \emph{decouple} the relatively simple problem of determining a ``pivot'' optimal EBM from the more difficult problem of exploiting this EBM at inference time, 
%an approach inspired by \citet{A-parshakova-etal-2019-global}, who applied a similar strategy to a different problem (improving the data-efficiency of autoregressive models over synthetic data). 
Such decoupling is helpful, because it permits to better diagnose the important challenges to focus on.
%
%\footnote{See \citep{A-parshakova-etal-2019-global} for a similar decomposition with a different objective.}  

% While most of the existing work on Controlled Generation has taken what we have called a \emph{pointwise} view: focusing on the quality of each individual output, as opposed to \emph{distributional} properties of the collection of all outputs. 

% And in fact, the standard objective of RL is to \emph{optimize} a pointwise reward. Policy-gradient methods do consider distributions over outputs, but only as a tool towards producing maximal rewards; and in fact, it is a side-effect of the limited capacity of the policy networks that such distributions do not peak on a single output, as would be the optimal outcome in cases of real-valued rewards with no ties.\footnote{In which cases the distribution $q$ maximizing $\E_{x\sim q} R(x)$ would be $q=\delta_{x^*}$ for $x^* = \argmax_x R(x)$.}
% %
% By contrast to this usual optimization ``intent'', our own intent here is explicitly distributional, and the policies we are looking for are not simply tools towards maximizing scores, but actual objectives in their own right.
% %
% Such a change of perspective might be argued against in the case of conditional seq2seq problems, such as Machine Translation, where focusing on a single good output for a given input makes sense,\footnote{By saying that, we do not imply that a distributional view does \emph{not} make sense also for conditional models, but this is a question that we leave for future work. \MD{hmmm?}} 
% but is clearly inadapted when focusing on language models.

%\footnote{In particular, it already allows to immediately compute the ratio $\frac{p(x_1)}{p(x_2}$ for arbitrary points $x_1, x_2$.}
%
%TBC TBC TBC TBC TBC TBC TBC TBC TBC TBC TBC TBC TBC TBC 

%It presents two serious issues. First, computing $Z$ can be challenging. Second, even if $Z$ were known, the ability to compute $p(x)$ exactly on each individual $x$ does not imply the ability to produce probabilistic samples from $p$.\footnote{The situation is comparable to optimization: being able to compute a score $v(x)$ for each $x$ does not imply the ability to find the maximum score.}

%One way to pin down a specific target distribution $p(x)$ consists in providing some ``prior" distribution $p_{prior}$, that is, a distribution that we would accept as our best guess if we did not have any specific ``expectations", and then to try and minimize the KL divergence $\KL(p, p_{prior})$ between our target distribution and the prior distribution, while respecting the moment constraints. Here, we take $p_{prior} = a(x) = \text{gpt-2}(x)$.

Note that in the case where the prior distribution would amount to total ignorance, that is, would be the uniform distribution over the sample space,\footnote{In the case of a uniform distribution, we have to assume a \emph{finite} discrete sample space.} then this approach would correspond to the well-known \emph{Maximum Entropy} technique \precite{MaxEnt}, a formal way of staying maximally noncommital to events while satisfying the expectation constraints.
In the general case of a non-uniform distribution 
%(over a general finite or infinite countable, or continuous, probability space.) 
the approach can be seen as a \emph{Generalized Maximum Entropy} principle (aka XXXX, YYYY), an approach which enjoys remarkable mathematical properties:\footnote{We gloss over certain details here, see section SSSS for more precise statements.}
\begin{enumerate}[nosep, left=0pt]
\item $p$ belongs to the \emph{exponential family} determined by $a$ and the vector  $\bphi(x) = (\phi_1(x),\ldots,\phi_k(x)) $ of features whose moments are constrained. In other words, $p$ can be expressed in the form $p(x) = 1/Z P(x)$, where $P(x) = a(x) \exp \langle \blambda, \bphi(x)\rangle$, for some vector of parameters $\blambda=(\lambda_1,\ldots,\lambda_k)$, and where $Z$ is a normalization constant.
\item The moment constraints then uniquely determine the value of the parameter vector $\blambda$, which can be efficiently obtained through a simple optimization procedure, leading to an explicit representation of $P$. We note that $P$ is an instance of an \emph{Energy Based Model} (EBM), namely an unnormalized distribution, and that the value of $Z$, is only determined \emph{implicitly} by the representation $P$.
\end{enumerate}

\fi %8-pages-constraint

==> sections/related.tex <==
\section{Related Work}

There is a large reinforcement-learning inspired literature about steering autoregressive models towards optimizing a task loss. \cite{seq_lvl_train_RanzatoCAZ15, BahdanauBXGLPCB17} use rewards based on BLEU and ROUGE for Machine Translation and Summarization. \cite{RL_dialogue_LiMRJGG16,RL_TambwekarDMMHR19} use heuristic rewards in order to improve certain a priori desirable features.  \\
%
When using such approaches, one should take care of not forgetting too much of the original LM policy (``degeneration''): \cite{LiuLSNCP16} noted that such optimization may produce poor examples that improve the average reward without an actual increase in readability or relevance. This has inspired previous work to rely on hand-crafted rewards to ensure the quality of generated text~\citep{Wu_googleMT16,PaulusXS18,gumbel_textgen_yang_NIPS2018}. \\
%
\cite{KL_Jaques17,KL_jaquesK19} and more recently \cite{Ziegler19} use a conservative fine-tuning approach with a KL penalty between the trained policy and the original auto-regressive model. This penalty acts as a regularizer that prevents the trained policy from deviating too much from the original policy.
%
Similarly, \cite{plug_and_play_20}, this time in a plug-and-play rather than a fine-tuning context, also use KL penalty, exploiting a noisy-channel objective combining the original policy with a task-related classifier. Noisy-channel was a popular technique in the early times of Statistical Machine Translation~\citep{Brown1994}, and gained renewed interest in an NMT context~\citep{fusion_StahlbergCS18,yu2019_noisychannel}.

Some of the previous approaches for combining the initial policy with controlling factors can be seen to involve, often implicitly, an EBM for which sequences of low energy are seeked. Some early NLP-related EBM research is concerned with sequence labelling problems (e.g. tagging) exploiting the global sequence \citep{andor_globally_2016,Belanger:2016:SPE:3045390.3045495}. More recently, \cite{A-parshakova-etal-2019-global} and \cite{Deng_EBM_20}, augment LMs with an additional global factor in order to get a lower perplexity on the training data. A recent survey of EBMs for text is \citep{Bakhtin2020EnergyBasedMF}. 

% But
One problem that is currently causing a lot of concern, and for which distributional control can be largely applied, is the problem of distributional biases apparent in LMs
\citep{bias_mt_stanovsky-etal-2019,bias_mt_PratesAL20,gpt3}.
%
However, little work so far has attempted solutions to the problem. \cite{BordiaB19} introduce a regularization term for reducing gender bias during training of a language model from scratch (as opposed to debiasing a pretrained model).
%
\cite{babysitter2_Sheng2020} introduce a method relying on adversarial triggers \citep{WallaceFKGS19}; this method does not de-bias the whole distribution but only obtains non-biased continuations of given prompts.\\
%
This previous work focuses on balancing between two specific demographics (e.g. gender); our approach allows to constrain the  expectations of any combination of binary or real-valued features, affording a flexible and formally clear way for controlling multiple constraints simultaneously.

